Temperature dependent fluctuations in the two-dimensional XY model

We present a detailed investigation of the probability density function (PDF) of order parameter fluctuations in the finite two-dimensional XY (2dXY) model. In the low temperature critical phase of this model, the PDF approaches a universal non-Gaussian limit distribution in the limit T-->0. Our analysis resolves the question of temperature dependence of the PDF in this regime, for which conflicting results have been reported. We show analytically that a weak temperature dependence results from the inclusion of multiple loop graphs in a previously-derived graphical expansion. This is confirmed by numerical simulations on two controlled approximations to the 2dXY model: the Harmonic and ``Harmonic XY'' models. The Harmonic model has no Kosterlitz-Thouless-Berezinskii (KTB) transition and the PDF becomes progressively less skewed with increasing temperature until it closely approximates a Gaussian function above T ~ 4\pi. Near to that temperature we find some evidence of a phase transition, although our observations appear to exclude a thermodynamic singularity.

==> figs/graphs_d.tex <==
%\documentclass[12pt]{article}
%\input{/home/simon/latex/mycommands}
%\usepackage{graphics}
%\usepackage{graphpap}
\newsavebox{\dotpair}
%\begin{document}
\begin{picture}(340,100)(0,0)
\thicklines
\savebox{\dotpair}(80,60)
{\dotty{0}{0}{10}
\dotty{0}{60}{10}}
\put(20,20){\usebox{\dotpair}}
\put(80,20){\usebox{\dotpair}}
\put(140,20){\usebox{\dotpair}}
\put(200,20){\usebox{\dotpair}}
\put(260,20){\usebox{\dotpair}}
\put(320,20){\usebox{\dotpair}}
\qbezier(20,20)(0,50)(20,80)
\qbezier(20,20)(40,50)(20,80)
\qbezier(80,20)(60,50)(80,80)
\qbezier(80,20)(100,50)(80,80)
\qbezier(140,20)(170,0)(200,20)
\qbezier(140,20)(170,40)(200,20)
\qbezier(140,80)(170,100)(200,80)
\qbezier(140,80)(170,60)(200,80)
\qbezier(260,20)(275.858,64.142)(320,80)
\qbezier(260,20)(304.142,35.858)(320,80)
\qbezier(320,20)(275.858,35.858)(260,80)
\qbezier(320,20)(304.142,64.142)(260,80)
\put(110,20){\Huge{,}}
\put(230,20){\Huge{,}}
\end{picture}
%\end{document}

